Pulsar radio emission mechanisms: a critique

We consider critically the three most widely favored pulsar radio emission mechanisms: coherent curvature emission (CCE), beam-driven relativistic plasma emission (RPE) and anomalous Doppler emission (ADE). We assume that the pulsar plasma is one dimensional (1D), streaming outward with a bulk Lorentz factor $\gamma_{\rm s} \gg \langle \gamma\rangle -1 \gtrsim 1$, where $\langle \gamma \rangle $ is the intrinsic spread in the rest frame of the plasma. We argue that the formation of beams in a multi-cloud model is ineffective in the intrinsically relativistic case for plausible parameters, because the overtaking takes too long. We argue that the default choice for the particle distribution in the rest frame is a J{\"u}ttner distribution and that relativistic streaming should be included by applying a Lorentz transformation to the rest-frame distribution, rather than the widely assumed relativistically streaming Gaussian distribution. We find that beam-driven wave growth is severely restricted by (a) the wave properties in pulsar plasma, (b) a separation condition between beam and background, and (c) the inhomogeneity of the plasma in the pulsar frame. The growth rate for the kinetic instability is much smaller and the bandwidth of the growing waves is much larger for a J{\"u}ttner distribution than for a relativistically streaming Gaussian distribution. No reactive instability occurs at all for a J{\"u}ttner distribution. We conclude that none of CCE, RPE and ADE in tenable as the generic pulsar radio emission mechanism for ``plausible'' assumptions about the pulsar plasma.

==> fig1a.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{005}[tc][tc]{\matlabtextA $ \gamma_{\rm s} $}%
\psfrag{006}[bc][bc]{\matlabtextA $ r/R_* $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{003}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{004}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>

==> fig1b.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{005}[tc][tc]{\matlabtextA $ \gamma_{\rm s} $}%
\psfrag{006}[bc][bc]{\matlabtextA $ r/R_* $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{003}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{004}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>

==> fig2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $ ck_{\parallel}/\omega_{\rm p}$}%
\psfrag{013}[bc][bc]{\matlabtextA $ \omega/\omega_{\rm p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $$}%
\psfrag{001}[ct][ct]{\matlabtextB $1$}%
\psfrag{002}[ct][ct]{\matlabtextB $$}%
\psfrag{003}[ct][ct]{\matlabtextB $2$}%
\psfrag{004}[ct][ct]{\matlabtextB $$}%
\psfrag{005}[ct][ct]{\matlabtextB $3$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> fig3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11}{11}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $ (1-z)/\rho^2 $}%
\psfrag{009}[bc][bc]{\matlabtextA $ \omega/\omega_{p} $}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.8$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.6$}%
\psfrag{002}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $\matlabfragNegXTick 0.2$}%
\psfrag{004}[ct][ct]{\matlabtextB $0$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> fig4.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $ r/R_* $}%
\psfrag{011}[bc][bc]{\matlabtextA $ \omega'_\pm/2\pi\, {\rm (GHz)} $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{2}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{4}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{6}$}%
%
%% </ytick>

==> figA2.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{11.00}{11.00}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextA $ x'/R_* $}%
\psfrag{015}[bc][bc]{\matlabtextA $ u'/u_i $}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10.00}{10.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $298$}%
\psfrag{001}[ct][ct]{\matlabtextB ${}$}%
\psfrag{002}[ct][ct]{\matlabtextB $298.4$}%
\psfrag{003}[ct][ct]{\matlabtextB ${}$}%
\psfrag{004}[ct][ct]{\matlabtextB $298.8$}%
\psfrag{005}[ct][ct]{\matlabtextB ${}$}%
\psfrag{006}[ct][ct]{\matlabtextB $299.2$}%
\psfrag{007}[ct][ct]{\matlabtextB ${}$}%
\psfrag{008}[ct][ct]{\matlabtextB $299.6$}%
\psfrag{009}[ct][ct]{\matlabtextB ${}$}%
\psfrag{010}[ct][ct]{\matlabtextB $300$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{013}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>
